The X-shooter Spectral Library (XSL): Data Release 3

We present the third data release (DR3) of the X-shooter Spectral Library (XSL). This moderate-to-high resolution, near-ultraviolet-to-near-infrared ($350-2480$ nm, R $\sim$ 10 000) spectral library is composed of 830 stellar spectra of 683 stars. DR3 improves upon the previous data release by providing the combined de-reddened spectra of the three X-shooter segments over the full $350-2480$ nm wavelength range. It also includes additional 20 M-dwarf spectra from the ESO archive. We provide detailed comparisons between this library and Gaia EDR3, MILES, NGSL, CaT library, and (E-)IRTF. The normalised rms deviation is better than $D=0.05$ or 5$\%$ for the majority of spectra in common between MILES (144 spectra of 180), NGSL (112$/$116), and (E-)IRTF (55$/$77) libraries. Comparing synthetic colours of those spectra reveals only negligible offsets and small rms scatter, such as the median offset(rms) 0.001$\pm$0.040 mag in the (box1-box2) colour of the UVB arm,-0.004$\pm$0.028 mag in (box3-box4) of the VIS arm, and -0.001$\pm$0.045 mag in (box2-box3) colour between the UVB and VIS arms, when comparing stars in common with MILES. We also find an excellent agreement between the Gaia published (BP-RP) colours and those measured from the XSL DR3 spectra, with a zero median offset and an rms scatter of 0.037 mag for 449 non-variable stars. The unmatched characteristics of this library, which combine a relatively high resolution, a large number of stars, and an extended wavelength coverage, will help us to bridge the gap between the optical and the near-IR studies of intermediate and old stellar populations, and to probe low-mass stellar systems.

==> Table_header.tex <==
%% Table: key dico
\begin{table*}
\caption{XSL keywords dictionary (primary header).}
{\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{l l l l  c}
\toprule\toprule
General topic & Data reduction step			& Keyword & 	Description  & Default value\\
\toprule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% General information
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{3}{2.5cm}{General information} & & OBJECT &  Machine-readable name of the star & \\
& & HNAME &  Human-readable name of the star & \\
& & XSL\_ID & X-shooter Spectral Library unique identifier & \\
%& & XSL\_NAME & Internal name for the science spectrum & \\
& & PROV\textit{i} & Originating raw science file(s) & \\
\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Data reduction
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 1D extraction
\multirow{12}{2.5cm}{Data reduction} & 1D extraction & EXT\_AVG & 	Two 1D-spectra averaged  & F \\
\cmidrule{2-5}
%% Response curve computation
%& Response curve	& CAL\_NAME & Internal name for the response curve used & \\
&  Response curve & CAL\_STAR & Spectro-photometric standard star target & \\
& & CAL\_RAW\textit{i} & Originating raw flux-standard file(s) & \\
\cmidrule{2-5}
%% Flux calibration
& First flux calibration  	& FLUX\_COR & 	First flux calibration applied & F \\
\cmidrule{2-5}
%% Flux-loss correction
& Flux-loss correction 	& LOSS\_COR & 	Correction for slit-losses applied in DR2 & F \\
& 	& SPL\_COR & 	Correction for slit-losses with a spline function applied in DR3  & F \\
%& & STA\_NAME & Internal name for the wide-slit spectrum used & \\
& & STA\_RAW\textit{i} & Originating raw wide-slit file(s) & \\
\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Other keywords
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Rest-frame correction
\multirow{15}{2.5cm}{Characterization and quality assurance}  & Rest-frame correction & REST\_COR & Correction to rest-frame applied & T\\
&                      & REST\_UVB & UVB $cz$ values$^{(1)}$ [in $\mathrm{km~s^{-1}}$]  & \\
&                      & REST\_VIS &VIS $cz$ values$^{(1)}$ [in $\mathrm{km~s^{-1}}$]  & \\
&                      & REST\_NIR &NIR $cz$ values$^{(1)}$ [in $\mathrm{km~s^{-1}}$]  & \\
\cmidrule{2-5}
%% Barycor values 
&   Barycor values & BARY\_COR & Barycentric radial velocity correction value & \\ 
\cmidrule{2-5}
%% Merging parameters 
&   Merging UVB, VIS, NIR spectra & S\_U\_VAL & UVB scaling factor value & \\ 
&& S\_U\_ORI & UVB scaling factor reference &\\
&& S\_N\_VAL & NIR scaling factor value &\\
&& S\_N\_ORI & NIR scaling factor origin reference &\\
&& ARM\_ZERO & DR2 arm spectrum missing (zeros) & F\\
\cmidrule{2-5}
%% Dust extinction values 
&   Galactic dust extinction & AV\_VAL & Total extinction in V & \\ 
&& AV\_ORI & AV origin reference (interp.;interp/spline;reference) & \\
\cmidrule{2-5}
%%%%%%%%%%%%%%%%%%%%%%%%
%% Quality flags -> UVB
& Quality flags &  SNR 	& 		Median signal-to-noise ratio & \\
\cmidrule{3-5}
% QC -> UVB
& & WAVY\_UVB &  	Wavy spectrum between 460 and 520 nm & F\\
& & &  	(suspected residuals of the blaze function) & \\
%& & WMIN\_UVB & 	Shortest useful wavelength [in nm]  & 300 \\ 
\cmidrule{3-5}
% QC -> VIS
& & HAIR\_VIS & Some narrow spikes in the VIS spectrum & F\\
& & NOIS\_VIS & Noisy VIS spectrum & F \\
& & WAVY\_VIS & Wavy in some part of the VIS spectrum  & F	 \\
\cmidrule{3-5}
% QC -> NIR
& & HAIR\_NIR & Some narrow spikes in the NIR spectrum & F \\
& & WAVY\_NIR & Wavy in some part of the NIR spectrum  & F	 \\
\bottomrule
\end{tabular}
}
\label{table:key_dico}
\\
} 
Notes to Table\,\ref{table:key_dico}. (1) The $cz$ values are barycentric.
\end{table*}

==> Table_pec_stars.tex <==
%-------------------------------------------------------------
% Peculiar stars or spectra
%\section{Comments about individual objects or spectra}
%\label{app:comments_stars}
%------------------------------------

\begin{table*}
\caption[]{Peculiar stars, abnormal spectra or zero spectrum.}
\label{tab:peculiar}
\centering
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{l| lll}
\toprule\toprule
Category & Spectrum (XSL\_ID) & Star (HNAME) & Comment \\ 
\toprule
%%%%%%%%%%%%%%%%%%
% PEC
%%%%%%%%%%%%%%%%%%
\multirow{16}{1.5cm}{Peculiar}  & X0085, X0133 & HD\,96446 & He-rich \\
&X0116 & HD\,57060 & P-Cygni emission in H$\alpha$ \& HeI (1.083$\mu$m); known eclipsing binary \\
&X0190 & OGLEII\,DIA\,BUL-SC19\,2332 & O-rich mira, possible TiO emission near 1.25\,$\mu$m \citep{LanconIAU18} \\
&X0214, X0248 & HD\,190073 & Herbig Ae/Be star, numerous emission lines, \\
  & & & continuum contribution from cool component in the NIR arm \\
&X0357 & CD-69\,1618 & He-rich \\
&X0420 & SV*\,HV\,11223 & S-star signatures confirmed \citep[ZrO, 940\,nm; cf.][]{WBF83} \\
&X0424 & CL*\,NGC\,6522\,ARP\,3213 & Superimposed stars with very different velocities: \\
&& & One dominant in the UVB arm  ($cz \simeq -198\,\mathrm{km\,s^{-1}}$), the other \\
 && & in the NIR ($cz \simeq +30\,\mathrm{km\,s^{-1}}$). The UVB velocity is used for the \\
 && & barycentric correction in all arms.\\
&X0513 & CL*\,NGC\,419\,LE\,35 & C-star with contamination by nearby hotter star below 450\,nm \\   
&X0653 & HD\,172488 & Possibly He-rich \\
&X0765 & SV*\,HV\,11366 & S-star signatures confirmed \citep[ZrO, 940\,nm; cf.][]{WBF83} \\
&X0798 & SHV\,0527122-695006 & M giant with contamination by nearby hot star below 450\,nm \\
\toprule
%%%%%%%%%%%%%%%%%%
%% Spectrum good but object name / spectral type discussion
%%%%%%%%%%%%%%%%%
\multirow{8}{1.5cm}{Spectral type discussion}  &X0478, X0675 & V874\,Aql & O-rich LPV (not C-star as was stated in \citealt{Nassau57}) \\
&X0587 & IRAS\,10151-6008? & O-rich star (not C-star as assumed in \citealt{Whitelock06}). \\
&& & We suspect Whitelock et al. observed 2MASS\,10165028-6023549, \\
&& & while we observed 2MASS\,10165173-6023466.\\
&X0660 & OGLE\,204664c4? & G8V/K0V star. This name was taken from \cite{Zoccali08}, \\
&& & but does not directly relate to the OGLE survey catalogs. \\
&& & Prefer Gaia DR2 4049054206130689024. \\
&X0876 & TU\,Car & O-rich LPV (as already suggested in \citealt{Aaronson89}), not C-star \\
\toprule
%%%%%%%%%%%%%%%%%%
%% Abnormal
%%%%%%%%%%%%%%%%%%
\multirow{15}{1.5cm}{Abnormal} & X0061 & SHV\,0525478-690944 & C star. NIR poor
below 1.3\,$\mu$m. \\
 &X0085 & HD\,96446 & Wavy NIR continuum (prefer X0133) \\ 
&X0144 & OGLEII\,DIA\,BUL-SC26\,0532 &  A few artificial waves in the VIS arm \\
& & & (residuals from stripes in raw images)\\
%
&X0196 & HD\,194453  & K-band continuum wavy \\
&X0208 & HD\,179821 & K-band continuum wavy \\
&X0214 & HD\,190073 & K-band continuum wavy (prefer X0248)\\
&X0221 & HD\,175640  & K-band continuum wavy \\ 
&X0237 & SHV\,0510004-692755 & A few artificial waves in the VIS arm, as for X0144. \\
&X0269 & HD\,163346 &  A few artificial waves in the VIS arm, as for X0144. \\
%&X0275 & HD\,204155 & wavy UVB and VIS arms (prefer X0179) \\ 
&X0304 & HD\,37828 & Continuum poor between 1 and 1.4\,$\mu$m (prefer X0097) \\ 
&X0338 & R~Cha & Slightly affected by saturation in the $H$-band [1600--1700 nm] \\
& & & and $K$-band  [2130--2230 nm] (NIR arm) \\
& X0450 & HD~166991 & Artifacts in $K$-band (NIR arm) \\
&X0758, X0766, X0790 & Feige\,110 & S/N ratio poor in NIR, use average \\
& X0778 & HD~11397 & Artifacts in $K$-band (NIR arm) \\
& X0834 & HD~42143 & Bad telluric correction (O$_2$) in $A$-band (VIS arm) \\
& X0878 & HD~83632 & Artifacts in $H$-band (NIR arm) \\
\toprule
%%%%%%%%%%%%%%%%%%
%% Parameters
%%%%%%%%%%%%%%%%%%
\multirow{8}{1.5cm}{Stellar param.$^{(1)}$} 
 %MD009 & HD\,31412B & From \citet{Terrien2015} \\
 %&MD002 & LTT\,2544 & From \citet{RAVE2017} \\
 %&MD021 & V*\,V645\,Cen & From\citet{Cenarro2007} \\ 
 &X0156 & GJ\,644C & From L20 \\
 &X0216, X0278 & HD\,216219 & From \citet{Cenarro2007} \\ 
 &X0243 & HD\,128801 & From \citet{Cenarro2007} \\ 
 &X0418 & HD\,2796 & From \citet{Cenarro2007} \\ 
 &X0430 & HD\,213042 & From \citet{Cenarro2007} \\ 
 &X0452 & HD\,179315 & From\citet{Luck2011} \\ 
 &X0754, X0755 & CL*\,NGC\,330\,ROB\,A3 & From \citet{Hill1999} \\ 

\toprule
\bottomrule
\end{tabular}
}
\end{table*}

%%%%%%%%%%%%%%%%%%
%% Zeros
%%%%%%%%%%%%%%%%%%
\begin{table*}
\caption[]{Zero spectrum}
\label{tab:peculiar2}
\centering
\resizebox{0.75\linewidth}{!}{
\begin{tabular}{l| lll}
\toprule\toprule
Category & Spectrum (XSL\_ID) & Star (HNAME) & Comment \\ 
\toprule
\multirow{15}{1.5cm}{Partially zero spectrum} 
& X0020 & ISO-MCMSJ005714.4-730121 & UVB \\
& X0029 &  ISO-MCMS J005304.7-730409 & UVB \\
& X0036 &  HD 39801 & NIR \\
& X0052 &  T Cae & NIR \\
& X0100 & SHV 0528537-695119 & UVB \\
& X0127 & CD-31 4916 & NIR \\
& X0130, X0131 & LHS 2065 & UVB \\
& X0145 & OGLEII DIA BUL-SC41 3443 & UVB \\
& X0150 & HD 101712 & NIR \\ 
& X0154 & BMB 286 & UVB \\ 	
& X0209	& GJ 752B & UVB \\
& X0233	& HD 165438 & NIR \\
& X0234 & IRAS 15060+0947 & NIR \\
& X0253 & OGLEII DIA BUL-SC22 1319 & UVB \\
& X0296 & OGLEII DIA BUL-SC13 0324 & UVB \\
& X0312	& HD 52005 & NIR \\
& X0316	& HD 76221 & NIR \\
& X0321	& HD 99648 & NIR \\
& X0330 & HD 35601 & NIR \\
& X0332	& BS 4463 & NIR \\
& X0336	& HD 63302 & NIR \\
& X0337	& RU Pup & NIR \\
& X0339	& HD 82734 & NIR \\
& X0340	& Y Hya & NIR \\
& X0341	& EV Car & NIR \\
& X0342	& BS 3923 & NIR \\
& X0343	& BS 4104 & NIR \\
& X0344	& CPD-5703502 & NIR \\
& X0353, X0605, X0606, X0635 &  [ABC89] Cir18 & UVB \\
& X0516 & SHV 0502469-692418 & UVB \\
& X0544	& SHV 0527072-701238 & UVB \\
& X0574	& [ABC89] Pup42 & UVB \\
& X0612 & HD 104307 & NIR\\
& X0653	& HD 172488 & UVB \\
& X0704	& NGC 6838 1037 & NIR \\
& X0759 &  HV\,12149 & UVB \\
& X0784 & SHV 0448341-691510 & NIR \\
& X0812 & SHV 0531398-701050 & NIR \\
& X0818, X0820 & SHV 0535237-700720& NIR \\
& X0830 & HD 36395 & NIR \\
& X0892	& LHS 318 & NIR \\	
\bottomrule
\end{tabular}
}

\end{table*}
